Clip-OGD: An Experimental Design for Adaptive Neyman Allocation in Sequential Experiments

From clinical development of cancer therapies to investigations into partisan bias, adaptive sequential designs have become increasingly popular method for causal inference, as they offer the possibility of improved precision over their non-adaptive counterparts. However, even in simple settings (e.g. two treatments) the extent to which adaptive designs can improve precision is not sufficiently well understood. In this work, we study the problem of Adaptive Neyman Allocation in a design-based potential outcomes framework, where the experimenter seeks to construct an adaptive design which is nearly as efficient as the optimal (but infeasible) non-adaptive Neyman design, which has access to all potential outcomes. Motivated by connections to online optimization, we propose Neyman Ratio and Neyman Regret as two (equivalent) performance measures of adaptive designs for this problem. We present Clip-OGD, an adaptive design which achieves $\widetilde{O}(\sqrt{T})$ expected Neyman regret and thereby recovers the optimal Neyman variance in large samples. Finally, we construct a conservative variance estimator which facilitates the development of asymptotically valid confidence intervals. To complement our theoretical results, we conduct simulations using data from a microeconomic experiment.

==> tex/old-comparison.tex <==

\subsection{Comparison to Explore-then-Commit} \label{sec:ec-comparison}


A popular experimental design for Adaptive Neyman Allocation is the two-stage design \citep{Hahn2011Adaptive, Blackwell2022Batch} which we call Explore-then-Commit, due to its similarities to algorithms in the bandits literature \citep{Lattimore2020Bandit}.
At a high level, an Explore-then-Commit design runs the Bernoulli design with $p = 1/2$ for $T_0 \leq T$ iterations, uses the collected data to estimate $p^*$ by $\widehat{p}^*$ and then runs the Bernoulli design with $p = \widehat{p}^*$ for the remaining $T_1 = T - T_0$ iterations.
This design is conceptually simpler than \ourdesign{} and may be used in more restricted settings where the experimental design permits only one adaptive change in treatment probabilities.
However, previous works have not been able to show it recovers the Neyman variance and \citet{Cai2022Performance} demonstrates that for small $T_0$, the Explore-then-Commit designs actually suffers increased variance relative to non-adaptive baselines.
We provide further negative results in this direction: in a design-based framework, for any $T_0$, there are outcomes satisfying Assumption~\ref{assumption:bounded-moments} for which Explore-then-Commit incurs (at least) linear expected Neyman regret.

\begin{proposition} \label{prop:EC-regret}
	\todo{FILL THIS IN}
\end{proposition}

The proof of Proposition~\ref{prop:EC-regret} and further discussion appear in Appendix~\todo{ref}.
The bad cases are essentially when the estimated $\widehat{p}^*$ may be very far from the true optimal probability $p^*$.
In a design-based setting, this can happen when the outcomes of units in the explore phase are not representative of the entire sequence.
Formulating conditions under which Explore-then-Commit designs achieve low Neyman regret is beyond the scope of this paper, but the proof of Proposition~\ref{prop:EC-regret} shows that regularity conditions on the order of the units will be required.
